PLVS: A SLAM System with Points, Lines, Volumetric Mapping, and 3D Incremental Segmentation

This document presents PLVS: a real-time system that leverages sparse SLAM, volumetric mapping, and 3D unsupervised incremental segmentation. PLVS stands for Points, Lines, Volumetric mapping, and Segmentation. It supports RGB-D and Stereo cameras, which may be optionally equipped with IMUs. The SLAM module is keyframe-based, and extracts and tracks sparse points and line segments as features. Volumetric mapping runs in parallel with respect to the SLAM front-end and generates a 3D reconstruction of the explored environment by fusing point clouds backprojected from keyframes. Different volumetric mapping methods are supported and integrated in PLVS. We use a novel reprojection error to bundle-adjust line segments. This error exploits available depth information to stabilize the position estimates of line segment endpoints. An incremental and geometric-based segmentation method is implemented and integrated for RGB-D cameras in the PLVS framework. We present qualitative and quantitative evaluations of the PLVS framework on some publicly available datasets. The appendix details the adopted stereo line triangulation method and provides a derivation of the Jacobians we used for line error terms. The software is available as open-source.

==> sections/lines.tex <==

% Internal convention:
% matrices: a matrix M is reported as $\textbf{M}$ []
% 2D vectors: a 2D vector v is reported as $\bm{v}$
% 3D vectors: a 3D vector P is reported as $\bm{P}$
% tuples: $(a,b,c)$
% sets: a set $\cal S$
% scalars: light lower case letters $s$
% ??? functions: (including images) by light upper case letters (I)

The architecture of the sparse SLAM system reflects the one of ORB-SLAM~\cite{mur2017orb, campos2021orb}. The extraction of keylines, the tracking, mapping and bundle-adjustment of 3D line segments proceed in parallel with the corresponding operations on keypoints and 3D points. Below, we provide futher details about management and representation of keylines and 3D line segments.

\subsection{Notation}

Throughout this paper, we use the following notation. $\Omega \subset \mathbb{R}^2$ is the image domain. The generic $i$-th RGB-D image $(I_i,D_i)$ consists of a rectified colour image $I_i: \Omega \rightarrow \mathbb{N}^3$ and a registered depth image $D_i: \Omega \rightarrow \mathbb{R}^+$. The depth image $D_i$ returns for each pixel $\bm{u}=[u,v]^T \in  \Omega$ the positive  distance between the image plane and the closest object point intercepted by the ray emanated from the camera center and passing through $\bm{u}$. 

The camera transformation matrix corresponding to $(I_i,D_i)$ is denoted by $\textbf{T}_i = \in SE(3)$, transforming a point
%an homogeneous point $\bar{\bm{P}} = [\bm{P},1]^T$ 
from the world frame to the camera frame. One has 
\begin{equation}
\textbf{T}_i = \begin{bmatrix}
       \textbf{R}_i &   \bm{t}_i       \\
       \textbf{0}^T & 1 
     \end{bmatrix}
\end{equation}
where $\textbf{R}_i \in SO(3)$ and $\bm{t}_i \in \mathbb{R}^3$. For 3D points, we use the superscripts $c$ and $w$ to indicate the camera and world frames in which point coordinates are expressed respectively. 

Given a vector $\bm{v}$, we define the vector $\widebar{\bm{v}} \triangleq [\bm{v}^T,1]^T$. 
%For instance, $\widebar{\bm{u}} = [\bm{u}^T,1]^T \in \mathbb{R}^3$ is the normalized homogeneous representation of $\bm{u}$. 
Moreover, we define  the operator $\bm{\gamma}: \mathbb{R}^3 \rightarrow \Omega$ as $\bm{\gamma}([u,v,w]^T)=[u/w,v/w]^T$. 
%It is used, for instance, to obtain $\bm{u} = \pi(\widebar{\bm{u}})$.  
%Its inverse operator is denoted by  $\pi^{-1}: \Omega \rightarrow \mathbb{R}^3$. It is $\pi^{-1}([x,y]^T)=[x,y,1]^T$.


Let $\textbf{K}\in \mathbb{R}^{3\times 3}$ be the fixed camera calibration matrix. The camera projection $\bm{u} \in  \Omega$ of a 3D point $\bm{P}^c = [x,y,z]^T \in \mathbb{R}^3$ is
\begin{equation}\label{eq:CameraProjection}
\bm{u} = \bm{\gamma}(\textbf{K} \bm{P}^c) = \Bigg[ f_x \frac{x}{z} + c_x, f_y \frac{y}{z} + c_y \Bigg]^T
\end{equation}
where $(f_x,f_y) \in \mathbb{R}^2$ defines the focal length and $(c_x,c_y) \in \mathbb{R}^2$ is the principal point. 

The 3D backprojection of a pixel $\bm{u} \in \Omega$ given the depth image $D_i$ is 
\begin{equation}\label{Eq:Backprojection}
\bm{P} = \textbf{K}^{-1}  \widebar{\bm{u}} D_i(\bm{u}) = \Bigg[ \frac{(u-c_x)}{f_x}\delta, \frac{(v-c_y)}{f_y}\delta, \delta \Bigg]^T
\end{equation}
where $\delta = D_i(\bm{u}) \in \mathbb{R}^+$. 

For an RBG-D image $(I_i,D_i)$, we define (with a slight abuse of notation) the projection map $\bm{\pi}_i : \mathbb{R}^3 \rightarrow \Omega $ and 
the backprojection map $\bm{\beta}_i :  \Omega \rightarrow \mathbb{R}^3$  as follows
\begin{equation}
\bm{\pi}_i(\bm{P}^w)\triangleq \bm{\gamma}(\textbf{K} [\textbf{R}_i,\bm{t}_i]\widebar{\bm{P}}^w),
\qquad \bm{\beta}_i(\bm{u}) = \textbf{K}^{-1}  \widebar{\bm{u}} D_i(\bm{u}).
\end{equation}

On the image plane, we consider 2D line equations of the following form 
\begin{equation}\label{Eq:LineEquation}
\bm{n}^T \bm{u} - h = 0 
\end{equation} 
where $\bm{n} = [n_u,n_v] \in \mathbb{R}^2$ is the unit normal direction and $h \in \mathbb{R}$ is the signed distance of the considered line from the origin. Given two points $\bm{u}_1, \bm{u}_2 \in \Omega$, we compute $\bm{n}=[\Delta v, -\Delta u]^T/\sqrt(\Delta^2 u + \Delta^2 v)$ and $h=\bm{n}^T\bm{u}_1$ (or $h=\bm{n}^T\bm{u}_2$).

Given a covariance matrix $\bm{\Sigma}  \in \mathbb{R}^{n \times n}$, the Mahalanobis distance between two vectors $\bm{v},\bm{w} \in \mathbb{R}^n$ is $\| \bm{v} - \bm{w}\|_{\bm{\Sigma}} = (\bm{v} - \bm{w})^T\bm{\Sigma}^{-1} (\bm{v} - \bm{w})$. We denote by $\bm{I}_n$ the identity matrix of size $n \times n$.


\input{sections/points}

\begin{figure}[!t]
\begin{center}
{\centering\includegraphics[scale=1]{figures/lines2.pdf}} \caption{The schema shows how three line segment observations $\{(\bm{p}_i,\bm{q}_i)\}_{i=1}^{3}$ of the same 3D line segment $l$ are  backprojected onto the 3D line at different elements of the class ${\cal C}_l$.
%The generic line segment $l$ with its corresponding representations.
} \label{Fig:LineRepresentation}
\end{center}
\end{figure}



\subsection{Line Segments Representation}

A 3D line segment $l$ is represented in the sparse map ${\cal M}_s$ by a pair of 3D endpoints $\bm{P}, \bm{Q} \in \mathbb{R}^3$. 
%$l$ is detected and matched in a subset of the acquired camera images. 
The detection of $l$ in an image (following a 2D line fitting stage) consists of a support region~\cite{ma2012invitation}, which is a 2D compact and connected region ${\cal W}(l) \subset \Omega$ represented  by two endpoints $\bm{p}_i,\bm{q}_i \in \Omega$. The matched pair of image endpoints $(\bm{p}_i,\bm{q}_i)$ is also referred to as the $i$-th \emph{line segment observation} of $l$.  

Due to noise, possible occlusions and other factors, the 3D line segment $l$ may not be fully observed by the camera. In fact, backprojecting all observations $\{(\bm{p}_i,\bm{q}_i)\}_{i=1}^{n_l}$ of $l$ one obtains a class of 3D line segments ${\cal C}_l =  \{(\bm{\beta}_i(\bm{p}_i),\bm{\beta}_i(\bm{q}_i)) \in \mathbb{R}^3 \times \mathbb{R}^3, i=1,...,n_l \}$ where, in general, $\| \bm{\beta}_i(\bm{p}_i) - \bm{\beta}_i(\bm{q}_i) \| \neq \| \bm{\beta}_j(\bm{p}_j) - \bm{\beta}_j(\bm{q}_j) \|$ for $i \neq j$ (see Fig.~\ref{Fig:LineRepresentation}). Here, for simplicity, we assumed the $i$-th observation $(\bm{p}_i,\bm{q}_i)$ occurs in the $i$-th image $(I_i,D_i)$. 

In general, we define the representation of a 3D line segment $l$ according to the following:
\begin{enumerate}
\item the 2D image endpoints $\bm{p}_i,\bm{q}_i \in \Omega$ in the generic image $(I_k,D_k)$ where $l$ is detected and successfully matched;
\item the 3D backprojected endpoints $\bm{\beta}_k(\bm{p}_i),\bm{\beta}_k(\bm{q}_i) \in \mathbb{R}^3$ \emph{attached} to the camera frame of $(I_k,D_k)$;
\item the 3D map endpoints $\bm{P}, \bm{Q} \in \mathbb{R}^3$ which represent the line segment $l$ in the map ${\cal M}_s$. 
\end{enumerate}
For simplicity, we do not explicit the implied mapping $k=k(i)$ which is built at extraction/matching time and associates the $i$-th observation of $l$ with the $k$-th frame/keyframe. 

A line segment observation $(\bm{p}_i,\bm{q}_i)$ is defined \emph{stereo} if both the depths $D_k(\bm{p}_i)$ and $D_k(\bm{q}_i)$ exist and are finite\footnote{Indeed, with commodity RGB-D sensors, the depth $D_i$ may be not defined for each pixel.}; \emph{mono} otherwise. 

Note that only a stereo observation allows to compute $\bm{\beta}_k(\bm{p}_i)$ and $\bm{\beta}_k(\bm{q}_i)$. Indeed, the availability of the 3D backprojected points allows to introduce a new type of error that takes into account depth information in order to  better estimate the position of line segment endpoints during bundle adjustment stages (see Sect.~\ref{Sect:ReprojectionErrors}). 

\luigi{As noted below, we can replace the 3D regularizer (\ref{Eq:3DDistancePointBackProjPoint}) with a 2D regularized which does not need any depth information.}

\subsection{Line Segments Detection and Matching}

\luigi{Insert figure for the detection and matching stages.}

For each processed image $I_i$, a Gaussian image pyramid is first computed. Then, line segments are extracted on each level of the image pyramid by using the EDlines method described in~\cite{akinlar2011edlines}. This consists in a linear time algorithm which also includes a false detection control. We selected the EDlines method for its repeatability, precision and efficiency. 
%real-time performances on a two-level image pyramid. 

On each level of the image pyramid, we model the uncertainty in the endpoints detection process with a specific noise variance. We denote by $\sigma^2_{li} \in \mathbb{R}$ the noise variance on each coordinate of the image endpoints $\bm{p}_i,\bm{q}_i$.
 
To attain frame-to-frame line matching, a binary descriptor is associated with each extracted line segment by using the Line Band Descriptor (LBD) method~\cite{zhang2013efficient}. 
%Hamming distance is used as metric in nearest neighbor searches. 

We use a tiling technique to speed up line segment matching. In particular, at extraction time, we compute for each line segment its normal orientation $\theta = {\rm atan2}(n_v,n_u)$ and signed distance $h$. We partition the 2D parameter space $(\theta,h)$ into tiles. As a consequence, for each image $I_i$, we group the extracted line segments into their corresponding tiles and store the resulting partition in~$I_i$.

At matching time, we first project a 3D line segment $l \in {\cal M}_s$ over the target image $I_i$; then, we compute its projected line representation $(\theta_l,h_l)$; subsequently, we identify as candidate matches of $l$ in $I_i$ all the line segments of $I_i$ whose parameters $(\theta,h)$ lie in the same tile. Finally, the identified candidate matches are scored according to the Hamming distances between their descriptors. In order to reject possible false matches, we validate a nearest neighbor if \emph{(i)} its Hamming distance ratio with respect to second-closest neighbor is below a certain threshold (in general $0.8$) \emph{(ii)} its line-segment to line-segment distance on the image plane is below a certain threshold (in general $40$ pixels).


\begin{figure}[!t]
\begin{center}
{\centering\includegraphics[scale=1.3]{figures/linesErrors.pdf}} \caption{The generic 3D line segment $l$, its obversation $(\bm{p}_i,\bm{q}_i)$ in the image $(I_k,D_k)$ and the map endpoints $(\bm{P},\bm{Q})$ with their camera projections $(\bm{p},\bm{q}) = (\bm{\pi}_k(\bm{P}),\bm{\pi}_k(\bm{Q}))$. The 2D reprojection error $e_{2D}$ in eq.~(\ref{Eq:2DReprojectionError}) combines the depicted perpendicular point-line distances of $\bm{p}$ and $\bm{q}$ from the line $(\bm{p}_i,\bm{q}_i)$. On the other hand, the 3D backprojection error $e_{3D}$ in eq.~(\ref{Eq:3DBackprojectionError}) combines \emph{(i)} the 3D perpendicular point-line distances of $\bm{P}$ and $\bm{Q}$ from the 3D line $(\bm{\beta}_k(\bm{p}_i),\bm{\beta}_k(\bm{q}_i))$  and \emph{(ii)} the 3D endpoint-endpoint distances $\|\bm{P}-\bm{\beta}_k(\bm{p}_i)\|$ and $\|\bm{Q}-\bm{\beta}_k(\bm{q}_i)\|$.} \label{Fig:LineErrors}
\end{center}
\end{figure}


\subsection{Line Reprojection and Backprojection Errors}\label{Sect:ReprojectionErrors}

In order to incorporate line segments into  Bundle Adjustement (BA) we need to define a proper line reprojection error and to compute its differential with respect to both camera pose parameters and 3D line segment parameters. 

Consider the generic line segment $l$ with its $n_l \in \mathbb{N}$ observations $\{(\bm{p}_i,\bm{q}_i)\}_{i=1}^{n_l}$ and its 3D representation $(\bm{P}, \bm{Q})$ in the sparse map ${\cal M}_s$. In BA, each observation $(\bm{p}_i,\bm{q}_i)$ matches $l$ in a precise keyframe $k$ whose camera transformation is $\textbf{T}_k$. 

Given the observation $(\bm{p}_i,\bm{q}_i)$, its equation parameters $(\bm{n}_i,h_i)$ follow from eq.~(\ref{Eq:LineEquation}). On the image plane, we compute the 2D distance  between the camera projection of a 3D point $\bm{X}^w \in \mathbb{R}^3$  and the 2D line passing through the points $\bm{p}_i$ and $\bm{q}_i$ as
\begin{equation}\label{Eq:2DDistancePointLineSegment}
d_{2D}(i,k,\bm{X}^w) \triangleq \bm{n}_i^T \bm{\pi}_k(\bm{X}^w) - h_i
\end{equation}
%Let $\textbf{L}^w \triangleq (\bm{P}^w, \bm{Q}^w)$ denote the pair of map endpoints expressed in world frame. 
We define the 2D line-line distance vector
\begin{equation}\label{Eq:2DDistanceMapPointsLineSegment}
\bm{d}_{2D}(i,k) \triangleq \begin{bmatrix}
      d_{2D}(i,k,\bm{P}^w) \\
      d_{2D}(i,k,\bm{Q}^w)
     \end{bmatrix} \in \mathbb{R}^2
\end{equation}
whose $2 \times 2$  covariance matrix covariance  matrix is
\begin{equation}\label{Eq:SigmaD2DLine}
\bm{\Sigma}_{li} =  
\begin{bmatrix}    
\sigma_{d2D}^2(i, k,\bm{P}^w) & 0 \\
 0  & \sigma_{d2D}^2(i, k,\bm{Q}^w)
 \end{bmatrix} \in \mathbb{R}^{2 \times 2}
\end{equation}
\begin{equation}
\sigma_{d2D}^2(i, k,\bm{X}^w) = \Scale[1]{ 
\frac{\partial d_{2D}}{\partial (\bm{p}_i,\bm{q}_i)}\sigma_{li}^2 \bm{I}_4           
\frac{\partial d_{2D}}{\partial (\bm{p}_i,\bm{q}_i)}^T
}
\in \mathbb{R}
\end{equation}
where $\frac{\partial d_{2D}}{\partial (\bm{p}_i,\bm{q}_i)} \in \mathbb{R}^{1 \times 4}$ is the Jacobian of eq.~(\ref{Eq:2DDistancePointLineSegment}) with respect to both image endpoints coordinates. Here, for simplicity, we imposed $\bm{\Sigma}_{li}$ is diagonal. 

  
Given a mono line segment observation, its 2D reprojection error is defined as
\begin{align}\label{Eq:2DReprojectionError}
e_{2D}^L(i, k) &\triangleq   \rho_{\tau_2} \bigg( \| \bm{d}_{2D}(i,k) \|_{\bm{\Sigma}_{li}}\bigg)
\end{align}
where $\rho_{\tau_2}$ is the robust Huber cost function~\cite{hartley2003multiple, huber2011robust} depending on the threshold parameter $\tau_2$ (see Sect.~\ref{Sect:ImplementationDetails}). 

It is worth noting that eq.~(\ref{Eq:2DReprojectionError}) combines the 2D point-line distances on the image plane as shown in Fig.~\ref{Fig:LineErrors}.
%perpendicular distances between the camera projections of $\bm{P}^w$ and $\bm{Q}^w$  and the 2D line passing through the points $\bm{p}_i$ and $\bm{q}_i$ (see Fig.~\ref{Fig:LineErrors}).
In our experimental analysis, we have verified that it is  more suitable to include in the BA process mono line segments with at least $n_l \geq 3$ observations. 
%In our approach, we include mono line segments in the BA process only if they have at least .  

Now, moving to 3D, 
%let $\bm{\beta}_i(\textbf{l}_i)   \triangleq (\bm{\beta}_i(\bm{p}_i), \bm{\beta}_i(\bm{q}_i))$ denote the pair of 3D backprojected endpoints. 
we define the following 3D distances
\begin{align}\label{Eq:3DDistancePointLineSegment}
d_{3D}(i, k, \bm{X}^w) &\triangleq \frac{\Vert (\bm{X}^c - \bm{\beta}_k(\bm{p}_i))\times (\bm{X}^c - \bm{\beta}_k(\bm{q}_i)) \Vert }{\Vert \bm{\beta}_k(\bm{p}_i) - \bm{\beta}_k(\bm{q}_i) \Vert } \\
\label{Eq:3DDistancePointBackProjPoint}
d_P(\bm{x}, k, \bm{X}^w) &\triangleq \Vert \bm{X}^c - \bm{\beta}_k(\bm{x}) \Vert \\
\label{Eq:CoordinatesFromWtoC}
\bm{X}^c &\triangleq \textbf{R}_k \bm{X}^w +\bm{t}_k
\end{align}
where  eq.~(\ref{Eq:3DDistancePointLineSegment}) represents the 3D perpendicular distance between the map point $\bm{X}$ and the 3D line $(\bm{\beta}_k(\bm{p}_i),\bm{\beta}_k(\bm{q}_i))$ (here $\bm{X}^w$ coordinates have been transformed to camera frame by using eq.~(\ref{Eq:CoordinatesFromWtoC})) and eq.~(\ref{Eq:3DDistancePointBackProjPoint}) represents the distance between $\bm{X}$ and the backprojection of its associated image point $\bm{x} \in \Omega$. 

\luigi{In principle, the 3D regularizer (\ref{Eq:3DDistancePointBackProjPoint}) could be replaced by a 2D regularized which constists of the 2D distance of the projection of $\bm{X}^c$ from $\bm{x}$. To be evaluated. }

Proceeding as above, we define the 3D distance vector
\luigi{Here we insert a scalar weight $\mu \in [0,1]$ for assigning a different importance to $d_P$. In general, we privelge minimizing $d_{3D}$ distances (i.e. $\mu < 1$).} 
\begin{equation}\label{Eq:3DDistanceBB}
\bm{d}_B(i, k) \triangleq \begin{bmatrix}
      d_{3D}(i, k,\bm{P}^w) + \mu d_P(\bm{p}_i, k,\bm{P}^w)\\
      d_{3D}(i, k,\bm{Q}^w) + \mu d_P(\bm{q}_i, k,\bm{Q}^w)
     \end{bmatrix} \in \mathbb{R}^2
\end{equation}
%and the 3D endpoint-endpoint distance vector as
%\begin{equation}\label{Eq:3DDistanceMapPointsPointSegment}
%\bm{d}_P(i, k) \triangleq \begin{bmatrix}
%      d_P(\bm{p}_i, k,\bm{P}^w) \\
%      d_P(\bm{q}_i, k,\bm{Q}^w)
%     \end{bmatrix} \in \mathbb{R}^2.
%\end{equation}
%We combine them in the backprojection distance vector $\bm{d}_B(i, k) = \bm{d}_{3D}(i, k) + \bm{d}_P(i, k)$ 
whose $2\times2$  covariance matrix is set as
\begin{equation}\label{Eq:SigmaLi}
\bm{\Sigma}_{Li} =  
\begin{bmatrix}
\sigma_{dB}^2(i, k,\bm{P}^w)          
& \bm{0} \\
\bm{0} & 
\sigma_{dB}^2(i, k,\bm{Q}^w)           
\end{bmatrix}  \in \mathbb{R}^{2 \times 2}
\end{equation}  
\begin{equation}\label{Eq:SigmaD3D}
\sigma_{dB}^2(i, k,\bm{X}^w) 
 \triangleq \\
\Scale[0.8]{
\textbf{J}_{dB}(\bm{X}^w)     
\begin{bmatrix}
\bm{\Sigma}_{\beta}(\bm{p}_i)          
& \bm{0} \\
\bm{0} & 
\bm{\Sigma}_{\beta}(\bm{q}_i)            
\end{bmatrix} 
\textbf{J}_{dB}(\bm{X}^w)^T
}    
\end{equation}
\begin{equation}\label{Eq:Jd3D}
\textbf{J}_{dB}(\bm{X}^w) \triangleq
\frac{\partial (d_{3D}(i, k,\bm{X}^w) + \mu d_{P}(\bm{x}_i, k,\bm{X}^w)) }{\partial (\bm{\beta}_k(\bm{p}_i),\bm{\beta}_k(\bm{q}_i))}\in \mathbb{R}^{1 \times 6}
\end{equation}
\begin{equation}\label{Eq:SigmaBeta1}
\bm{\Sigma}_{\beta}(\bm{x}) \triangleq
\Scale[0.9]{\frac{\partial \bm{\beta}_k(\bm{x})}{\partial (u,v,\delta)} }         
\Scale[0.9]{\begin{bmatrix}
       \sigma_{li}^2 & 0 & 0 \\
       0 & \sigma_{li}^2 & 0 \\       
       0 & 0 & \sigma_{z}^2(\delta)  
     \end{bmatrix}} \Scale[0.9]{\frac{\partial \bm{\beta}_k(\bm{x})}{\partial (u,v,\delta)} ^T} 
     \in \mathbb{R}^{3 \times 3}
\end{equation}
where  $\textbf{J}_{dB}(\bm{X}^w) \in \mathbb{R}^{1 \times 6}$ is the Jacobian of eq.~(\ref{Eq:3DDistancePointLineSegment}) with respect to the coordinates of both the backprojected endpoints $\bm{\beta}_k(\bm{p}_i)$ and $\bm{\beta}_k(\bm{q}_i)$, $\frac{\partial \bm{\beta}_k(\bm{x})}{\partial (u,v,\delta)} \in \mathbb{R}^{3 \times 3}$ is the Jacobian of eq.~(\ref{Eq:Backprojection}) with respect to $u,v,\delta$. It is worth noting that \textit{(i)} for simplicity, we imposed $\bm{\Sigma}_{Li}$ is diagonal  \textit{(ii)} $\bm{\Sigma}_{\beta}(\bm{x}_i)$ represents the (induced) noise covariance matrix of the 3D backprojected point $\bm{\beta}_k(\bm{x})$. 

For a stereo line observation, we define the following 3D \emph{backprojection error} as
\begin{align}\label{Eq:3DBackprojectionError}
e_{3D}^L(i, k) &\triangleq   \rho_{\tau_3}\bigg( \|
\bm{d}_B(i, k) \|_{\bm{\Sigma}_{Li}}  \bigg).
\end{align}
Note that the backprojection error combines the 3D line-line distances and the 3D endpoint-endpoint distances as illustrated in Fig.~\ref{Fig:LineErrors}. 

In the appendix, we sketch how to compute the differentials of the reprojection and backprojection errors along with their covariance matrices. 

It is worth noting that in order to properly compute the distances $d_P$ (which are combined in the backprojection error~(\ref{Eq:3DBackprojectionError})), we need to properly associate $\bm{\beta}_k(\bm{p}_i)$ with $\bm{P}^w$ and $\bm{\beta}_k(\bm{q}_i)$ with $\bm{Q}^w$. This can be achieved during BA initialization by computing the distances between the two candidate pairings $(\bm{\beta}_k(\bm{p}_i),\bm{P}^c)$ and $(\bm{\beta}_k(\bm{p}_i),\bm{Q}^c)$ and then associating the closest pairs of points.

\luigi{The second term $d_P$ acts as a regularization term which naturally constraints the parametrization (otherwise the end-points would run away along the lines) and allow to obtain better configured representations end-points.}

Indeed, minimizing the 3D backprojection error of eq.~(\ref{Eq:3DBackprojectionError}) has two effects: \textit{(i)} aligning in each camera frame the 3D map line segment $(\bm{P},\bm{Q})$ to its corresponding backprojected line segment $(\bm{\beta}_k(\bm{p}_i),\bm{\beta}_k(\bm{q}_i))$ by taking into account the available depth information (cfr. eq~(\ref{Eq:3DDistancePointLineSegment})) \textit{(ii)} keep each 3D map endpoint $\bm{P}$ $(\bm{Q}$) close as much as possible to the centroid of all its backprojected representations $\bm{\beta}_k(\bm{p}_i)$ ($\bm{\beta}_k(\bm{q}_i)$) (cfr. eq~(\ref{Eq:3DDistancePointBackProjPoint}) and refer to Fig.~\ref{Fig:LineErrors}).


\subsection{Sparse Map Bundle Adjustment}

The back-end of the sparse SLAM uses \emph{full} Bundle Adjustment (BA) in order to compute  an optimal estimate of the model parameters in the sparse map ${\cal M}_s$. These are the poses of the keyframes $\cal K$, the positions of the 3D feature points  $\cal P$ and the 3D endpoint positions of the line segments $\cal L$. On the other hand, \emph{local} BA optimizes only the model parameters of points, line segments and poses corresponding to a set of keyframes which are covisible with the current reference keyframe~\cite{mur2017orb}. 

In BA, the optimality of the estimates is implicitly defined by the reprojection errors which are minimized. Under a suitable mathematical formulation, BA is equivalent to a MAP or MLE estimation depending on the presence of a prior~\cite{cadena2016past, hartley2003multiple}. 

The complete objective function which is minimized by full BA is
\begin{align}\label{Eq:FullObjectiveFunInBA}
E &\triangleq \underset{k \in {\cal K}}{\sum} \Bigg( \underset{i \in {\cal P}^m_k}{\sum} e_{2D}^P(i, k) + \underset{h \in {\cal P}^s_k}{\sum} e_{3D}^P(h, k) +  \nonumber \\ 
&\quad \underset{j \in {\cal L}^m_k}{\sum} e^L_{2D}(j, k)  + \underset{r \in {\cal L}^s_k}{\sum} \Big( e^L_{2D}(r, k)  + e^L_{3D}(r, k) \Big) \Bigg)
\end{align}
where ${\cal K}$ is the set of keyframes, ${\cal P}^x_k \subset {\cal P}$ and ${\cal L}^x_k \subset {\cal L}$ are respectively the subsets of points and line segments which are observed  in the $k$-th keyframe, and the superscript $x \in \{m,s\}$ denotes mono or stereo observations.  

The optimization is performed by using the Levenberg-Marquardt method, where the augmented normal equations 
\begin{equation}
(\textbf{J}^T \bm{\Sigma}^{-1} \textbf{J} + \lambda \textbf{I}) \Delta \bm{\theta} =  -\textbf{J}^T\bm{\Sigma}^{-1} \bm{e}
\end{equation}
are iteratively solved in order to obtain the udpate of the full vector $\bm{\theta}$ of map parameters. Here, the error vector $\bm{e}$ combines all the reprojection and backprojection errors included in eq.~(\ref{Eq:FullObjectiveFunInBA}), and $\bm{\Sigma}$ combines all the corresponding covariance matrices.


\begin{figure}[!t]
\begin{center}
{\centering\includegraphics[scale=0.25]{figures/maps-without-with-backprojection-error.png}} \caption{Two 3D maps of line segments built for the same enviroment. \emph{Left}: the map built without using the backprojection error. \emph{Right}: map obtained by including the backprojection error in BA.} \label{Fig:MapsWithoutWithBackprojErrors}
\end{center}
\end{figure}


Note that we introduced the 3D backprojection error~(\ref{Eq:3DBackprojectionError}) since we observed that the 2D line reprojection errors~(\ref{Eq:2DReprojectionError}) are not enough to stabilize the position estimates of the 3D line segment endpoints $\bm{P}^w_j, \bm{Q}^w_j \in {\cal M}_s$. Indeed, with reference to Fig.~\ref{Fig:LineRepresentation}, one can easily figure out that, in the ideal case the camera projections of $\bm{P}^w$ and $\bm{Q}^w$ perfectly lie on the observed image lines segments $(\bm{p}_i,\bm{q}_i)$, the 2D line reprojection errors do not change if $\bm{P}^w$ and $\bm{Q}^w$ shift along their 3D line direction.

In practice, many experiments confirmed that  without the use of the 3D backprojection errors, the positions of the 3D line segment endpoints $\bm{P}^w_j, \bm{Q}^w_j$ usually drift along the line directions and the estimate of the line directions tends to degrade. In most cases, the line-segment-culling remove many unstable line segments from ${\cal M}_s$ after a couple of frames, since these do not succeed to find a proper match anymore. Indeed, this observed issue deserved a solution since it cancel out most of the benefits of including line segments in the sparse SLAM. Fig.~\ref{Fig:MapsWithoutWithBackprojErrors} shows two maps of the same environment obtained with and without including the backprojection error in BA. 


==> sections/tables.tex <==
\begin{table*}[t]
\begin{adjustbox}{width=\textwidth} 
\begin{tabular}{l|c|c|c}
Dataset& PLVS-RMSE &ElasticFusion-RMSE & FrameDrops \\
\midrule
freiburg1 360 & 0.095& 0.108&  1.6\% \\
freiburg1 desk & 0.015& 0.02&  3.1\% \\
freiburg1 desk2 & 0.039& 0.048&  3.2\% \\
freiburg1 floor &  - &  - &  11.8\% \\
freiburg1 plant & 0.019& 0.022&  1.3\% \\
freiburg1 room & 0.058& 0.068&  0.7\% \\
freiburg1 rpy & 0.018& 0.025&  4.0\% \\
freiburg1 teddy & 0.043& 0.083&  1.3\% \\
freiburg1 xyz & 0.009& 0.011&  0.8\% \\
freiburg2 360 hemisphere & 0.144&  - &  2.2\% \\
freiburg2 360 kidnap &  - &  - &  1.2\% \\
freiburg2 coke & 0.511&  - &  2.0\% \\
freiburg2 desk & 0.013& 0.071&  2.5\% \\
freiburg2 dishes & 0.032&  - &  2.2\% \\
freiburg2 large no loop & 0.525&  - &  1.8\% \\
freiburg2 large with loop &  - &  - &  2.4\% \\
freiburg2 metallic sphere & 0.721&  - &  1.7\% \\
freiburg2 metallic sphere2 & 0.121&  - &  1.2\% \\
freiburg2 pioneer 360 &  - &  - &  61.6\% \\
freiburg2 pioneer slam &  - &  - &  52.7\% \\
freiburg2 pioneer slam2 &  - &  - &  52.3\% \\
freiburg2 pioneer slam3 &  - &  - &  32.3\% \\
freiburg2 rpy & 0.003& 0.015&  2.1\% \\
freiburg2 xyz & 0.006& 0.011&  1.5\% \\
freiburg3 cabinet &  - &  - &  4.1\% \\
freiburg3 large cabinet & 0.043& 0.099&  3.9\% \\
freiburg3 long office household & 0.011& 0.017&  4.9\% \\
freiburg3 nostructure notexture far &  - &  - &  4.7\% \\
freiburg3 nostructure notexture near withloop &  - &  - &  3.9\% \\
freiburg3 nostructure texture far & 0.031& 0.074&  4.0\% \\
freiburg3 nostructure texture near withloop & 0.022& 0.016&  3.5\% \\
freiburg3 structure notexture far & 0.021& 0.03&  3.5\% \\
freiburg3 structure notexture near & 0.02& 0.021&  3.7\% \\
freiburg3 structure texture far & 0.011& 0.013&  4.7\% \\
freiburg3 structure texture near & 0.015& 0.015&  4.9\% \\
freiburg3 teddy &  - & 0.049&  4.2\% \\


\end{tabular}
\end{adjustbox}
\caption{ATE RMSE and STD on the evaluated static scene datasets of ~\cite{sturm12iros}, using always the same parameters. Although the capturing device provides RGB-D frames at 30Hz, a number of sequences are missing a certain amount of frames that were simply never recorded. This value is represented in FrameDrops column. This percentage is provided by ~\cite{whelan2016elasticfusion}.}
\label{Tab:trackAcc}
\end{table*}











































\begin{table*}[t]
\begin{adjustbox}{width=\textwidth} 
\begin{tabular}{l|cc|cc|c|c}
Dataset & PLVS-P-RMSE & PLVS-P-LOST & PLVS-PL-RMSE & PLVS-PL-LOST & ElasticFusion-RMSE & FrameDrops \\
\midrule
freiburg1 360 & 0.209709 & 0 & 0.095676 & 0 & 0.108 & 1.6\% \\
freiburg1 desk & 0.01561 & 2 & 0.015792 & 0 & 0.02 & 3.1\% \\
freiburg1 desk2 & 0.02302 & 1 & 0.039633 & 0 & 0.048 & 3.2\% \\
freiburg1 floor & - & 5 & - & 5 & - & 11.8\% \\
freiburg1 plant & 0.014714 & 0 & 0.020575 & 0 & 0.022 & 1.3\% \\
freiburg1 room & 0.063147 & 0 & 0.06036 & 0 & 0.068 & 0.7\% \\
freiburg1 rpy & 0.021416 & 0 & 0.018436 & 0 & 0.025 & 4.0\% \\
freiburg1 teddy & - & 4 & 0.043727 & 1 & 0.083 & 1.3\% \\
freiburg1 xyz & 0.009729 & 0 & 0.009692 & 0 & 0.011 & 0.8\% \\
freiburg2 360 hemisphere & - & 4 & 0.144988 & 1 & - & 2.2\% \\
freiburg2 360 kidnap & - & 5 & - & 5 & - & 1.2\% \\
freiburg2 coke & - & 4 & 0.510676 & 1 & - & 2.0\% \\
freiburg2 desk & 0.008305 & 0 & 0.013404 & 0 & 0.071 & 2.5\% \\
freiburg2 dishes & 0.043513 & 0 & 0.032529 & 0 & - & 2.2\% \\
freiburg2 large no loop & 0.210336 & 0 & 0.525601 & 0 & - & 1.8\% \\
freiburg2 large with loop & - & 3 & - & 3 & - & 2.4\% \\
freiburg2 metallic sphere & - & 5 & 0.721055 & 0 & - & 1.7\% \\
freiburg2 metallic sphere2 & 0.227863 & 2 & 0.121611 & 0 & - & 1.2\% \\
freiburg2 pioneer 360 & - & 5 & - & 5 & - & 61.6\% \\
freiburg2 pioneer slam & - & 5 & - & 5 & - & 52.7\% \\
freiburg2 pioneer slam2 & - & 5 & - & 5 & - & 52.3\% \\
freiburg2 pioneer slam3 & - & 5 & - & 5 & - & 32.3\% \\
freiburg2 rpy & 0.00312 & 0 & 0.003056 & 0 & 0.015 & 2.1\% \\
freiburg2 xyz & 0.003798 & 0 & 0.006609 & 0 & 0.011 & 1.5\% \\
freiburg3 cabinet & - & 5 & - & 5 & - & 4.1\% \\
freiburg3 large cabinet & - & 3 & 0.043743 & 0 & 0.099 & 3.9\% \\
freiburg3 long office household & 0.010322 & 0 & 0.011873 & 0 & 0.017 & 4.9\% \\
freiburg3 nostructure notexture far & - & 5 & - & 5 & - & 4.7\% \\
freiburg3 nostructure notexture near withloop & - & 5 & - & 5 & - & 3.9\% \\
freiburg3 nostructure texture far & 0.043296 & 0 & 0.030099 & 0 & 0.074 & 4.0\% \\
freiburg3 nostructure texture near withloop & 0.022714 & 0 & 0.022261 & 0 & 0.016 & 3.5\% \\
freiburg3 structure notexture far & 0.038519 & 0 & 0.021302 & 0 & 0.03 & 3.5\% \\
freiburg3 structure notexture near & 0.023198 & 0 & 0.020095 & 2 & 0.021 & 3.7\% \\
freiburg3 structure texture far & 0.010575 & 0 & 0.011232 & 0 & 0.013 & 4.7\% \\
freiburg3 structure texture near & 0.01057 & 0 & 0.015167 & 0 & 0.015 & 4.9\% \\
freiburg3 teddy & - & 5 & - & 4 & 0.049 & 4.2\% \\

\end{tabular}
\end{adjustbox}
\caption{ATE RMSE and STD on the evaluated static scene datasets of ~\cite{sturm12iros}, using always the same parameters. Although the capturing device provides RGB-D frames at 30Hz, a number of sequences are missing a certain amount of frames that were simply never recorded. This value is represented in FrameDrops column. This percentage is provided by ~\cite{whelan2016elasticfusion}.}
\label{Tab:trackAcc}
\end{table*}
































\begin{table*}[t]
%\centering
%\Scale[0.9]{
%\footnotesize{
%\scalebox{0.7}{}
%\renewcommand{\arraystretch}{0.75} 
%\resizebox{\linewidth}{!}{%
\begin{adjustbox}{width=\textwidth} 
\begin{tabular}{l|ccccccc}
%\toprule
Dataset & P RMSE & P STD & P LOST & PL RMSE & PL STD & PL LOST & FrameDrops \\
\midrule
freiburg1 360 & 0.209709 & 0.031187 & 0 & 0.095676 & 0.004862 & 0 & 1.6\% \\
freiburg1 desk & 0.01561 & 0.000375 & 2 & 0.015792 & 0.00014 & 0 & 3.1\% \\
freiburg1 desk2 & 0.02302 & 0.006284 & 1 & 0.039633 & 0.005567 & 0 & 3.2\% \\
freiburg1 floor & - & - & 5 & - & - & 5 & 11.8\% \\
freiburg1 plant & 0.014714 & 0.000728 & 0 & 0.020575 & 0.001882 & 0 & 1.3\% \\
freiburg1 room & 0.063147 & 0.009955 & 0 & 0.06036 & 0.008011 & 0 & 0.7\% \\
freiburg1 rpy & 0.021416 & 0.000873 & 0 & 0.018436 & 0.000647 & 0 & 4.0\% \\
freiburg1 teddy & - & - & 4 & 0.043727 & 0.008643 & 1 & 1.3\% \\
freiburg1 xyz & 0.009729 & 0.000236 & 0 & 0.009692 & 0.00011 & 0 & 0.8\% \\
freiburg2 360 hemisphere & - & - & 4 & 0.144988 & 0.014651 & 1 & 2.2\% \\
freiburg2 360 kidnap & - & - & 5 & - & - & 5 & 1.2\% \\
freiburg2 coke & - & - & 4 & 0.510676 & 0.0352 & 1 & 2.0\% \\
freiburg2 desk & 0.008305 & 0.001883 & 0 & 0.013404 & 0.001682 & 0 & 2.5\% \\
freiburg2 dishes & 0.043513 & 0.004488 & 0 & 0.032529 & 0.001175 & 0 & 2.2\% \\
freiburg2 large no loop & 0.210336 & 0.082454 & 0 & 0.525601 & 0.142543 & 0 & 1.8\% \\
freiburg2 large with loop & - & - & 3 & - & - & 3 & 2.4\% \\
freiburg2 metallic sphere & - & - & 5 & 0.721055 & 0.030826 & 0 & 1.7\% \\
freiburg2 metallic sphere2 & 0.227863 & 0.043679 & 2 & 0.121611 & 0.021812 & 0 & 1.2\% \\
freiburg2 pioneer 360 & - & - & 5 & - & - & 5 & 61.6\% \\
freiburg2 pioneer slam & - & - & 5 & - & - & 5 & 52.7\% \\
freiburg2 pioneer slam2 & - & - & 5 & - & - & 5 & 52.3\% \\
freiburg2 pioneer slam3 & - & - & 5 & - & - & 5 & 32.3\% \\
freiburg2 rpy & 0.00312 & 0.000111 & 0 & 0.003056 & 0.000129 & 0 & 2.1\% \\
freiburg2 xyz & 0.003798 & 0.000094 & 0 & 0.006609 & 0.000125 & 0 & 1.5\% \\
freiburg3 cabinet & - & - & 5 & - & - & 5 & 4.1\% \\
freiburg3 large cabinet & - & - & 3 & 0.043743 & 0.004109 & 0 & 3.9\% \\
freiburg3 long office household & 0.010322 & 0.000891 & 0 & 0.011873 & 0.001288 & 0 & 4.9\% \\
freiburg3 nostructure notexture far & - & - & 5 & - & - & 5 & 4.7\% \\
freiburg3 nostructure notexture near withloop & - & - & 5 & - & - & 5 & 3.9\% \\
freiburg3 nostructure texture far & 0.043296 & 0.007088 & 0 & 0.030099 & 0.002103 & 0 & 4.0\% \\
freiburg3 nostructure texture near withloop & 0.022714 & 0.002572 & 0 & 0.022261 & 0.005248 & 0 & 3.5\% \\
freiburg3 structure notexture far & 0.038519 & 0.018329 & 0 & 0.021302 & 0.001741 & 0 & 3.5\% \\
freiburg3 structure notexture near & 0.023198 & 0.00853 & 0 & 0.020095 & 0.00196 & 2 & 3.7\% \\
freiburg3 structure texture far & 0.010575 & 0.000489 & 0 & 0.011232 & 0.001214 & 0 & 4.7\% \\
freiburg3 structure texture near & 0.01057 & 0.001471 & 0 & 0.015167 & 0.002967 & 0 & 4.9\% \\
freiburg3 teddy & - & - & 5 & - & - & 4 & 4.2\% 
%\bottomrule
\end{tabular}
%}
\end{adjustbox}
\caption{ATE RMSE and STD on the evaluated static scene datasets of ~\cite{sturm12iros}, using always the same parameters. Although the capturing device provides RGB-D frames at 30Hz, a number of sequences are missing a certain amount of frames that were simply never recorded. This value is represented in FrameDrops column. This percentage is provided by ~\cite{whelan2016elasticfusion}.}
\label{Tab:trackAcc}
\end{table*}

\begin{table*}[t]
\begin{adjustbox}{width=\textwidth} 
\begin{tabular}{l|cc|cc|c|c}
Dataset & PLVS-P-RMSE & PLVS-P-LOST & PLVS-PL-RMSE & PLVS-PL-LOST & ElasticFusion & FrameDrops 
\midrule
freiburg1 360 & 0.209709 & 0 & 0.095676 & 0 & 0.108 & 1.6\% \\
freiburg1 desk & 0.01561 & 2 & 0.015792 & 0 & 0.02 & 3.1\% \\
freiburg1 desk2 & 0.02302 & 1 & 0.039633 & 0 & 0.048 & 3.2\% \\
freiburg1 floor & - & 5 & - & 5 & - & 11.8\% \\
freiburg1 plant & 0.014714 & 0 & 0.020575 & 0 & 0.022 & 1.3\% \\
freiburg1 room & 0.063147 & 0 & 0.06036 & 0 & 0.068 & 0.7\% \\
freiburg1 rpy & 0.021416 & 0 & 0.018436 & 0 & 0.025 & 4.0\% \\
freiburg1 teddy & - & 4 & 0.043727 & 1 & 0.083 & 1.3\% \\
freiburg1 xyz & 0.009729 & 0 & 0.009692 & 0 & 0.011 & 0.8\% \\
freiburg2 360 hemisphere & - & 4 & 0.144988 & 1 & - & 2.2\% \\
freiburg2 360 kidnap & - & 5 & - & 5 & - & 1.2\% \\
freiburg2 coke & - & 4 & 0.510676 & 1 & - & 2.0\% \\
freiburg2 desk & 0.008305 & 0 & 0.013404 & 0 & 0.071 & 2.5\% \\
freiburg2 dishes & 0.043513 & 0 & 0.032529 & 0 & - & 2.2\% \\
freiburg2 large no loop & 0.210336 & 0 & 0.525601 & 0 & - & 1.8\% \\
freiburg2 large with loop & - & 3 & - & 3 & - & 2.4\% \\
freiburg2 metallic sphere & - & 5 & 0.721055 & 0 & - & 1.7\% \\
freiburg2 metallic sphere2 & 0.227863 & 2 & 0.121611 & 0 & - & 1.2\% \\
freiburg2 pioneer 360 & - & 5 & - & 5 & - & 61.6\% \\
freiburg2 pioneer slam & - & 5 & - & 5 & - & 52.7\% \\
freiburg2 pioneer slam2 & - & 5 & - & 5 & - & 52.3\% \\
freiburg2 pioneer slam3 & - & 5 & - & 5 & - & 32.3\% \\
freiburg2 rpy & 0.00312 & 0 & 0.003056 & 0 & 0.015 & 2.1\% \\
freiburg2 xyz & 0.003798 & 0 & 0.006609 & 0 & 0.011 & 1.5\% \\
freiburg3 cabinet & - & 5 & - & 5 & - & 4.1\% \\
freiburg3 large cabinet & - & 3 & 0.043743 & 0 & 0.099 & 3.9\% \\
freiburg3 long office household & 0.010322 & 0 & 0.011873 & 0 & 0.017 & 4.9\% \\
freiburg3 nostructure notexture far & - & 5 & - & 5 & - & 4.7\% \\
freiburg3 nostructure notexture near withloop & - & 5 & - & 5 & - & 3.9\% \\
freiburg3 nostructure texture far & 0.043296 & 0 & 0.030099 & 0 & 0.074 & 4.0\% \\
freiburg3 nostructure texture near withloop & 0.022714 & 0 & 0.022261 & 0 & 0.016 & 3.5\% \\
freiburg3 structure notexture far & 0.038519 & 0 & 0.021302 & 0 & 0.03 & 3.5\% \\
freiburg3 structure notexture near & 0.023198 & 0 & 0.020095 & 2 & 0.021 & 3.7\% \\
freiburg3 structure texture far & 0.010575 & 0 & 0.011232 & 0 & 0.013 & 4.7\% \\
freiburg3 structure texture near & 0.01057 & 0 & 0.015167 & 0 & 0.015 & 4.9\% \\
freiburg3 teddy & - & 5 & - & 4 & 0.049 & 4.2\% \\
%\bottomrule
\end{tabular}
\end{adjustbox}
\caption{ATE RMSE and STD on the evaluated static scene datasets of ~\cite{sturm12iros}, using always the same parameters. Although the capturing device provides RGB-D frames at 30Hz, a number of sequences are missing a certain amount of frames that were simply never recorded. This value is represented in FrameDrops column. This percentage is provided by ~\cite{whelan2016elasticfusion}.}
\label{Tab:trackAcc}
\end{table*}
